Evaluating Low-Power Wireless Cyber-Physical Systems

Simulation tools and testbeds have been proposed to assess the performance of control designs and wireless protocols in isolation. A cyber-physical system (CPS), however, integrates control with network elements, which must be evaluated together under real-world conditions to assess control performance, stability, and associated costs. We present an approach to evaluate CPS relying on embedded devices and low-power wireless technology. Using one or multiple inverted pendulums as physical system, our approach supports a spectrum of realistic CPS scenarios that impose different requirements onto the control and networking elements. Moreover, our approach allows one to flexibly combine simulated and real pendulums, promoting adoption, scalability, repeatability, and integration with existing wireless testbed infrastructures. A case study demonstrates implementation, execution, and measurements using the proposed evaluation approach.

==> futureWork.tex <==
% !TEX root = paper.tex

\section{Future Work}
\label{sec:futureWork}

After having shown that we are able to control a real-world \cps over a multi-hop wireless network
we next want to investigate also synchronization tasks. For synchronization we will start with every
pendulum being stabilized by its own local controller, which can run with a high frequency due to
the wired connections, but for the synchronization task we need the wireless network. That way we
can manually adapt the difficulty of the control task by designing more ore less challenging
trajectories the carts have to follow. In synchronization tasks we explicitly benefit from the
inherent capability of \lwb to carry out many-to-many communication. If we want to synchronize two
or more pendulums, they need to know at least the actual state estimate of the leading pendulum. In
this setting we also want to demonstrate the advantages of event-based methods~\cite{Tr16,Tr17}.

Additionally to separately showing the ability of our network and controller for synchronization and
stabilization we also want to combine these tasks. As we have already experienced how challenging it
is to stabilize a pendulum over a multi-hop network it is not clear yet, if the combination of
stabilization and synchronization is possible.

